RPC Considered Harmful: Fast Distributed Deep Learning on RDMA

Deep learning emerges as an important new resource-intensive workload and has been successfully applied in computer vision, speech, natural language processing, and so on. Distributed deep learning is becoming a necessity to cope with growing data and model sizes. Its computation is typically characterized by a simple tensor data abstraction to model multi-dimensional matrices, a data-flow graph to model computation, and iterative executions with relatively frequent synchronizations, thereby making it substantially different from Map/Reduce style distributed big data computation. RPC, commonly used as the communication primitive, has been adopted by popular deep learning frameworks such as TensorFlow, which uses gRPC. We show that RPC is sub-optimal for distributed deep learning computation, especially on an RDMA-capable network. The tensor abstraction and data-flow graph, coupled with an RDMA network, offers the opportunity to reduce the unnecessary overhead (e.g., memory copy) without sacrificing programmability and generality. In particular, from a data access point of view, a remote machine is abstracted just as a "device" on an RDMA channel, with a simple memory interface for allocating, reading, and writing memory regions. Our graph analyzer looks at both the data flow graph and the tensors to optimize memory allocation and remote data access using this interface. The result is up to 25 times speedup in representative deep learning benchmarks against the standard gRPC in TensorFlow and up to 169% improvement even against an RPC implementation optimized for RDMA, leading to faster convergence in the training process.

==> discussion.tex <==
%!TEX root = main.tex
\section{Discussion}
\label{sec:discuss}
\subsection{Static Placement vs. Dynamic Allocation}
The tensor transfer mechanism with dynamic allocation incurs additional overhead compared to the mechanism with static placement; for example, due to the extra transfer of tensor meta-data and the on-demand tensor memory allocation. However, the dynamic mechanism does have some benefit with respect to reduced memory footprint because the receiver side memory allocated to tensor data can be freed when no longer needed in the subsequent computation. This saving can be critical in some scenarios, especially when tensors are stored in GPU memory. 

The memory consumption caused by the static placement may also introduce scalability issues. In distributed deep learning, parameter server~\cite{petuum15,ParameterServerLi2014} is a common architecture to support the computation. This is also the case in \tf{}, where partitions of the parameters (represented as variable tensors) of a neural network model are stored in a process that behaves as a parameter server. In this process, multiple sub-graphs associated with sessions initiated from different worker processes are executed in parallel and share those variable tensors. This means that there will be a \texttt{Recv} operator corresponding to a variable tensor for each worker to accept the model update from the worker. Therefore, the number of such tensors is proportional to the number of workers, so is the corresponding memory consumption, if the placement of the output tensor of the \texttt{Recv} operator is arranged statically. To address this issue, we enhance the graph analyzer to identify whether the tensor at the receiver end will be passed to a \texttt{Variable} operator, and if so, it only employs the transfer mechanism with dynamic tensor allocation.
